Toward Understanding Bugs in Vector Database Management Systems

Vector database management systems (VDBMSs) play a crucial role in facilitating semantic similarity searches over high-dimensional embeddings from diverse data sources. While VDBMSs are widely used in applications such as recommendation, retrieval-augmented generation (RAG), and multimodal search, their reliability remains underexplored. Traditional database reliability models cannot be directly applied to VDBMSs because of fundamental differences in data representation, query mechanisms, and system architecture. To address this gap, we present the first large-scale empirical study of software defects in VDBMSs. We manually analyzed 1,671 bug-fix pull requests from 15 widely used open-source VDBMSs and developed a comprehensive taxonomy of bugs based on symptoms, root causes, and developer fix strategies. Our study identifies five categories of bug symptoms, with more than half manifesting as functional failures. We further reveal 31 recurring fault patterns and highlight failure modes unique to vector search systems. In addition, we summarize 12 common fix strategies, whose distribution underscores the critical importance of correct program logic. These findings provide actionable insights into VDBMS reliability challenges and offer guidance for building more robust future systems.

==> Sections/2.related_work.tex <==
\section{Background and Related Work}
\label{related work}

\subsection{Vector Database Management Systems (VDBMSs)}

VDBMSs manage and retrieve high-dimensional vectors derived from unstructured data such as text, images, and audio. As shown in \autoref{fig:VDBMS}, they commonly adopt a client–server architecture: the server handles vector storage, indexing, and similarity search, while the client exposes interfaces for querying, data insertion, and metadata operations.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.95\linewidth]{Figures/VDBMS.pdf} 
    \caption{Architecture of VDBMSs.}
    \label{fig:VDBMS}
\end{figure}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/methodology.pdf} 
    \caption{Overview of the methodology for investigating bug characteristics in VDBMSs.}
    \label{fig:methodology}
\end{figure*}


\subsubsection{VDBMS Server}
User requests, transmitted via the client, flow through three layers on the server: query, index, and storage. The query layer parses and plans the request, the index layer performs efficient vector retrieval, and the storage layer provides access to the underlying data, which is then returned to the query layer for final processing and response.

\noindent\textbf{Query.} 
This layer includes four main components: operators, queries, the query optimizer, and the query executor. Operators perform tasks like similarity computation and result filtering, supporting query types such as k-nearest neighbor (k-NN)~\cite{Nearest-neighbor}, approximate search~\cite{ANN1993}, and range queries. For advanced use cases, it supports hybrid queries~\cite{wu2022hqann}, which combine vector similarity with attribute filters, and multi-vector queries, where multiple vectors and aggregated scores represent a single entity. The query optimizer selects efficient execution strategies, which are then carried out by the query executor through interaction with other VDBMS layers.

\noindent\textbf{Index.}  
The index layer is designed to accelerate similarity search over large collections of high-dimensional vectors by building specialized data structures that efficiently narrow down candidate results during query execution. Various indexing strategies can be employed, including table-based methods such as locality-sensitive hashing (LSH)~\cite{Muja2009}, tree-based approaches like random projection trees~\cite{NIPS2010_3def184a}, and graph-based structures such as HNSW~\cite{malkov2018efficient}.

\noindent\textbf{Storage.} 
This layer is responsible for managing all persistent data in the system, including vector embeddings, structured attributes, index files, and metadata. Its primary function is to ensure reliable storage and retrieval of this information while supporting efficient updates and access for query processing.



\subsubsection{VDBMS Client}
The client acts as the interface between users or applications and the VDBMS server. Most systems provide multi-language client SDKs, commonly written in Python, Java, Go, and JavaScript, which facilitate integration across diverse platforms. Some VDBMSs also offer graphical user interfaces to enhance client-side interaction; for example, Milvus provides a dedicated visual client called Attu~\cite{Attu}. Clients typically support two main communication protocols: REST APIs for lightweight metadata and control operations, and gRPC~\cite{grpc2025} for high-performance data transfer, particularly when handling large batches of vectors.

VDBMSs are essential for LLM applications using high-dimensional embeddings, providing core infrastructure for storing, searching, and managing vector data. They enable similarity-based retrieval for tasks like recommendation, anomaly detection, and semantic search, and also support RAG by supplying external knowledge to improve LLM responses.


\subsection{Reliability of VDBMSs}

The reliability of traditional DBMSs has long been a central topic of research. Liu~\ea~\cite{liu2024empiricalstudycharacteristicsdatabase} conducted a comprehensive analysis of 423 database access bugs across seven large-scale Java applications, while Cui~\ea~\cite{cui2024} examined 140 transaction-related bugs in six widely used database systems. Rigger~\ea~\cite{Rigger_2020} further introduced the Non-Optimizing Reference Engine Construction (NoREC) method to detect optimization bugs in query engines. These studies collectively reveal that DBMSs are susceptible to reliability issues stemming from diverse sources, including server-client interfacing, transaction handling, and query optimization.

In contrast, VDBMSs introduce a new set of reliability challenges due to their fundamental reliance on high-dimensional and semantically rich embeddings. Unlike traditional databases that operate over structured and ordinal data, VDBMSs must process unstructured data where query semantics are often ill-defined~\cite{tagliabue2023vectorspacefinalfrontier}. Moreover, the computational cost of vector comparisons is significantly higher, and building efficient yet consistent index structures for such data remains difficult~\cite{Wang2021,Wei2020,guo2022manucloudnativevector}. The complexity further increases with hybrid queries that integrate vector similarity with attribute-based filtering, complicating both query planning and execution. Although recent work has introduced various techniques to improve system efficiency, such as quantization-based compression~\cite{Gray,jegou2011,ite_matsui_2018} and learned partitioning methods~\cite{wang2017surveylearninghash,Muja2009,silpa2008}, these approaches largely focus on performance optimization. They offer limited solutions to deeper reliability concerns, such as incorrect results, inconsistent index states, or unpredictable behavior under dynamic workloads.
Given the growing use of VDBMSs in critical LLM applications, addressing their reliability challenges is both urgent and essential. This motivates our investigation into how these systems behave in practice and what factors underlie their failures.

==> Sections/4.statistical_results.tex <==
\section{Taxonomy and Patterns}
\label{statistical results}

This section reports our empirical analysis of 1,463 real-world bug-fixing PRs in VDBMSs, examining symptoms, root causes, and fix strategies according to the following research questions (RQs).

\noindent\hangindent=2.5em\hangafter=1\textbf{RQ1 What are the typical symptoms exhibited by bugs in VDBMSs, and how are they distributed?}
We identify common bug symptoms in VDBMSs, analyze their frequency and diversity, and examine how they reflect different severity levels across categories.

\noindent\hangindent=2.5em\hangafter=1\textbf{RQ2 What are the most bug-prone components in VDBMSs, and what are the key root causes?}
We analyze the distribution of bugs across VDBMS components, categorize their types, and identify all root causes.

\noindent\hangindent=2.5em\hangafter=1\textbf{RQ3 What fix strategies are commonly adopted for different types of bugs in VDBMSs?}
We analyze how developers fix bugs by identifying common strategies and their association with different bug types.

\subsection{RQ1: Symptoms.}
Based on our observations, the symptoms were grouped into five major categories as shown in \autoref{fig:symptom}. These categories capture the diverse ways in which bugs can manifest, ranging from critical disruptions such as system crashes to less severe but still impactful issues like misleading log messages or incorrect documentation.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{Figures/symptom.pdf}
    \caption{Distribution of symptoms.}
    \label{fig:symptom}
\end{figure}

\subsubsection{Crash}

Crash is the most severe symptom observed in VDBMSs, as it directly causes service termination and loss of availability. Crash-related bugs account for 15.1\% of all symptoms in our dataset, with the highest proportions found in Qdrant (40.7\%) and txtai (40\%), indicating these systems are particularly prone to critical failures. In VDBMSs, crashes typically manifest as abrupt process terminations, segmentation faults, or unrecoverable runtime exceptions. These symptoms are frequently observed in core components such as storage backends, query pipelines, and system integration layers. Compared to traditional DBMSs, VDBMSs are more susceptible to crash bugs due to their reliance on high-performance native libraries (e.g., BLAS, Faiss) and complex vector algorithms, which increase the risk of memory errors and environment-dependent failures. The greater algorithmic complexity and varied deployment scenarios in VDBMSs also make edge-case crashes harder to test, reproduce, and diagnose.


\begin{insightbox}
To reduce crash risks, VDBMS developers should test edge cases, abnormal inputs (e.g., NaN or out-of-bound vectors), and concurrency. Components written in low-level languages like C or C++ require particular attention due to their vulnerability to memory errors.
\end{insightbox}

\subsubsection{Functional Failure}
This is the most common symptom in our dataset, accounting for 57.3\% of all cases. These bugs cause incorrect behaviors such as inaccurate query results, missing search matches, inconsistent indexing outputs, or invalid status responses. They often stem from logical inconsistencies or algorithmic flaws in query processing and indexing, which are highly complex and sensitive to semantic similarity definitions. For example, a functional bug in Faiss was triggered by misconfigured IVF search parameters, producing ``-1'' placeholder IDs in top-k results. Since vector queries rely on approximate similarity and complex indexes like quantized or graph-based ANN structures, result correctness is especially vulnerable to logic bugs in similarity projection or quantization. Fixing these issues typically requires major changes to logic or data flow.

\begin{insightbox}
Robust functional testing in VDBMSs should target both typical and edge-case query scenarios, with particular emphasis on validating the logic and parameter handling of approximate search and indexing algorithms.
\end{insightbox}

\subsubsection{Performance Degradation}
Performance bugs comprise 7.3\% of all cases, typically manifesting as excessive resource use, slow response times, or throughput bottlenecks. These often result from inefficient indexes, misconfigured parameters, or suboptimal query execution. For example, in Vespa (PR \#31,664), a linear-weight ranking profile with a high hits value caused nodes to process too many documents, significantly slowing queries. Unlike crashes or functional failures, performance degradation is usually gradual and workload-dependent.



\subsubsection{Deployment Failure}
Deployment failures in VDBMSs typically occur during build, installation, or startup phases. Common symptoms include missing dependencies, incompatible compiler versions, broken build scripts, and misconfigured environment variables. These issues account for 10.2\% of cases in our dataset and are often amplified by reliance on specialized native libraries (e.g., BLAS, Faiss, SIMD) and integration with containerization frameworks. Unlike runtime failures, deployment bugs can prevent system launch, posing a major barrier to adoption, especially for new users and in CI/CD environments. Robust and portable deployment processes are essential for improving VDBMS reliability.


\begin{insightbox}
VDBMS developers should ensure portability and environment isolation by using containerized builds, automated installation scripts, and pre-check tools to detect missing dependencies or incompatible settings.
\end{insightbox}

\subsubsection{Logging \& Documentation Fault}
This category accounts for 10.1\% of all recorded symptoms and includes missing, misleading, or outdated logs and documentation. Faulty logging may obscure root causes by omitting key runtime information, while poor documentation, such as incorrect usage examples or missing configuration guidance, hinders adoption and usage. For VDBMSs with complex queries and configurations, clear logs and up-to-date documentation are essential for troubleshooting and user onboarding.


\begin{figure*}[h!]
    \centering
    \begin{subfigure}{0.95\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/classification_query_2.pdf}
        \caption{Classification result for bugs in \textit{Query}.}
        \label{fig:classification-query}
    \end{subfigure}
    
    \begin{subfigure}{0.95\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/classification_storage.pdf}
        \caption{Classification result for bugs in \textit{Storage}.}
        \label{fig:classification-storage}
    \end{subfigure}
    
    \begin{subfigure}{0.95\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/classification_parsing-interaction.pdf}
        \caption{Classification result for bugs in \textit{Parsing \& Interaction}.}
        \label{fig:classification-parsing_interaction}
    \end{subfigure}
    
    
    \begin{subfigure}{0.65\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{Figures/classification_index.pdf}
        \caption{Classification result for Index.}
        \label{fig:classification-index}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.30\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{Figures/classification_configuration.pdf}
        \caption{Classification result for Configuration.}
        \label{fig:classification-configuration}
    \end{subfigure}

    \caption{Overview and example of the bug classification method.}
    \label{fig:classification}
\end{figure*}
\subsection{RQ2: Root Causes.}
We construct a three-level taxonomy to classify bugs in VDBMSs, as shown in \autoref{fig:classification}. The percentages indicate the distribution of bugs at each level of the taxonomy. This taxonomy includes five categories: \textbf{Query} (711 bugs), \textbf{Storage} (182 bugs), \textbf{Index} (58 bugs), \textbf{Parsing \& Interaction} (125 bugs), and \textbf{Configuration} (387 bugs).


\subsubsection{Query} 
\label{subsub:query}
Query is the most bug-prone component, comprising 48.6\% of all cases. \textbf{\textit{Query algorithm logic issues}} (45.7\%) reflect challenges in ensuring correct query execution. \textbf{\textit{Query coordination issues}} (23.3\%) involve failures in managing concurrent execution and synchronization. \textbf{\textit{API interface issues}} (15.0\%) result from miscommunication between external APIs and internal handlers, while \textbf{\textit{memory management issues}} (8.7\%) stem from improper memory allocation or release during query processing.



\noindent\textbf{Query Algorithm Logic Issues.}
Incomplete or faulty logic in query algorithms, particularly when edge cases or unexpected inputs are overlooked, commonly leads to these bugs. \textbf{\textit{Missing exception handling mechanisms}}, such as failing to check for empty or null fields, which can lead to crashes. \textbf{\textit{Parameter misconfigurations}}, using illegal or ill-typed arguments, often result in subtle inaccuracies. \textbf{\textit{Data computation errors}}, like miscalculating similarity scores or buffer lengths, directly affect query reliability. \textbf{\textit{Filter abnormality}} refers to incomplete or incorrect filtering, causing improper inclusion or exclusion of data. These issues reflect the complexity of vector query logic and the challenge of anticipating all corner cases.


\begin{insightbox}
Ensuring the reliability of query algorithms in VDBMS requires thorough boundary testing and exception handling to address edge cases and unexpected parameter configurations.
\end{insightbox}

\noindent\textbf{Query Coordination Issues.}

Coordinating query stages or handling concurrent sessions can introduce subtle, hard-to-detect failures. One cause is \textbf{\textit{non-conformant data}}, where mismatched formats or inconsistent encoding disrupt execution. For example, in Weaviate (PR \#1,421), omitting the \texttt{\_additional} field led to incomplete downstream outputs. \textbf{\textit{State synchronization errors}} occur when components use outdated or inconsistent states, such as failing to terminate after a shutdown signal. \textbf{\textit{High-concurrency resource contention}} arises in parallel workloads, where poor thread or resource management results in race conditions, deadlocks, or degraded performance. Achieving reliable coordination requires consistent data interfaces, accurate state tracking, and careful concurrency control, which is particularly challenging in asynchronous and distributed VDBMS environments.

\noindent\textbf{API Interface Issues.}

System instability can arise from surface-level interfaces. \textbf{\textit{Parameter validation and handling errors}} occur when servers fail to verify input completeness, type, format, or range, or when dependencies and defaults are not properly enforced, leading to unexpected query behaviors. Another cause is \textbf{\textit{data transformation and response issues}}, often due to serialization or deserialization errors. For example, in Vespa (PR \#29,449), a misconfigured Jackson ObjectMapper resulted in malformed JSON during request parsing and response generation.
VDBMSs commonly process complex, nested queries with embeddings and hybrid parameters, where minor inconsistencies in input or response formatting can propagate system-wide. Robustness requires not just basic validation, but schema-aware design to ensure semantic consistency throughout the query lifecycle.


\noindent\textbf{Memory Management Issues.}  
High-dimensional vector computations introduce irregular, data-dependent memory access patterns that often lead to subtle memory errors.  
A common issue is \textbf{\textit{insufficient handling of boundary conditions}}, where the system fails to guard against edge cases such as buffer overflows or null pointer dereferences. For example, complex expressions evaluated over input vectors without proper checks can cause out-of-bounds access and crashes.  
Memory bugs also stem from \textbf{\textit{incorrect allocation strategies}}, including inaccurate memory estimation or poorly timed release. Premature deallocation can trigger use-after-free errors, while delayed release may cause memory leaks or bloat.  
In VDBMSs, memory usage is hard to predict due to factors like vector dimensionality, batch size, and filter complexity. To meet low-latency demands, systems often reuse buffers aggressively, increasing the risk of lifetime violations. These challenges are amplified by the large, high-dimensional nature of vector data, which is typically allocated in batches.


\begin{insightbox}
Memory allocation and usage in VDBMSs must account for the inherent complexity of vector data and various boundary conditions. The high dimensionality of vectors, coupled with data-dependent access patterns, demands precise memory estimation to avoid issues.
\end{insightbox}



\subsubsection{Storage}
As shown in \autoref{fig:classification-storage}, a total of 182 bugs are associated with the storage layer. These fall into two main categories: \textbf{\textit{Storage resource management issues}} (54.2\%), which concern the efficient utilization of storage resources and their impact on overall system performance; and \textbf{\textit{Storage data processing issues}} (41.2\%), which arise during data transformation, migration, or maintenance operations.



\noindent\textbf{Storage Data Processing Issues.}
VDBMSs are prone to data handling faults during storage operations, especially when serialization logic or validation mechanisms are poorly designed.  
\textbf{\textit{Serialization/Deserialization errors}} arise from mismatched formats, missing fields, or incompatible schema versions, leading to failures in persisting or restoring data. In some cases, valid data is rejected or causes crashes during deserialization.  
\textbf{\textit{Missing or faulty validation}} allows incorrect or corrupted records to enter the database, affecting downstream operations.  
\textbf{\textit{Missing exception handling}} can also hinder recovery from abnormal events. For example, in Milvus (PR \#36,149), the system failed to restore data after a crash, while in pgvecto.rs (PR \#242), a power loss left the database unrecoverable due to insufficient fault-tolerance logic.  
Unlike traditional DBMSs with well-defined schemas, VDBMSs often store high-dimensional data and index metadata in custom formats. This increases the risk of serialization mismatches, validation gaps, and deserialization errors, highlighting the need for specialized testing techniques.


\begin{insightbox}
Testing VDBMSs requires going beyond conventional strategies by incorporating various data schema fault injections to ensure robustness across heterogeneous and evolving data formats.
\end{insightbox}

\noindent\textbf{Storage Resource Management Issues.} 
Efficient storage resource utilization is critical in VDBMSs. 
In addition to the previously mentioned causes in \autoref{subsub:query}, such as \textbf{\textit{insufficient handling of boundary conditions}} and \textbf{\textit{high-concurrency resource contention}}, two other root causes are particularly relevant in this context. The first is \textbf{\textit{storage quota mechanism errors}}, where flawed strategies for allocating storage space, such as incorrect sharding logic, result in data being stored or retrieved incorrectly. The second is \textbf{cache not timely cleared}, where improper cache management, such as the failure to release memory after use, can lead to performance degradation or even system instability under sustained workloads.
Existing VDBMSs have adopted several practical strategies to optimize storage resource management, such as vector compression methods. However, our results show that bugs related to this category still account for 54.4\% of all storage-related issues. 

\begin{insightbox}
Stress testing VDBMS should focus on high-concurrency workloads, large-scale data ingestion, and edge cases like irregular sharding to ensure robust storage resource management under real-world conditions.
\end{insightbox}


\subsubsection{Parsing \& Interaction}
According to~\autoref{fig:classification-parsing_interaction}, 125 bugs are attributed to the parsing and interaction layer, stemming from client input parsing, result interpretation, and user-system interaction.
\textbf{\textit{Data handling issues}} (52\%), including failures in input parsing, format interpretation, and memory management during request and response processing.
\textbf{\textit{Permission configuration issues}} (25.6\%) involve authentication and access control, where misconfigurations result in failed or insecure interactions.  
\textbf{\textit{Resource and task management issues}} (18.4\%) concern incorrect memory allocation, poor task coordination, and errors in asynchronous execution.


\noindent\textbf{Data Handling Issues.}  
Data pipelines in VDBMSs are often fragile, breaking during request parsing or response reconstruction.  
A key root cause is \textbf{\textit{missing exception handling}}, where the system fails to detect or recover from malformed inputs, leading to crashes or undefined behavior.  
Another common issue is \textbf{\textit{data format parsing errors}}, caused by deviations from expected input structures, resulting in parsing failures or silent corruption.  
Response deserialization errors also occur when fields are missing, mismatched, or incompatible with the schema expected by the client.  
These failures highlight the need for defensive parsing strategies, such as schema validation, input fuzzing, and fallback mechanisms, to improve robustness against faulty inputs.


\noindent\textbf{Permission Configuration Issues.}
These issues mainly stem from \textbf{\textit{authentication mechanism errors}} or \textbf{\textit{authorization management errors}}. Authentication failures involve flawed user verification, allowing unauthorized access or blocking legitimate users. Authorization errors arise from misconfigured access rules, which can block valid actions or expose sensitive operations.
Such problems are critical in VDBMSs, which need fine-grained permissions for tasks like collection access, embedding uploads, and index changes. Operating in machine-to-machine environments or integrating with larger platforms, these systems are prone to subtle permission bugs from inconsistent roles, token scopes, or default settings.


\begin{insightbox}
Permission bugs in VDBMSs can block legitimate users or expose sensitive operations to unauthorized clients. Regular audits of configuration files and role definitions help detect misconfigurations early and ensure access controls align with intended security policies.
\end{insightbox}


\noindent\textbf{Resource and Task Management Issues.}  
The stability of VDBMSs often relies on careful control of memory usage and asynchronous task execution.
\textbf{\textit{Memory allocation errors}} occur when memory is allocated incorrectly, either too little or too much, during parsing or interaction, leading to performance issues or crashes. \textbf{\textit{Task management errors}} result from background operations that are not properly scheduled or monitored, causing inconsistent behavior.
For example, in LanceDB (PR \#407), a misconfigured timer led to irregular task execution and incorrect results. Robust VDBMSs require strict memory bounds, controlled asynchronous task lifecycles, and integrated observability mechanisms to detect anomalies early. These capabilities help prevent minor issues from propagating into major system failures.


\subsubsection{Index}
As shown in \autoref{fig:classification-index}, the Index aspect accounts for 58 bugs, representing only 4.0\% of the total. These are categorized into two types: \textbf{\textit{index construction and storage issues}}, which occur during index building, persistence, or updates; and \textbf{\textit{index usage issues}}, which arise during query execution using the index.
Despite their small number, indexing bugs can significantly affect system behavior. Structural or usage flaws may propagate to other components, resulting in incorrect queries or failures in data operations. As such, they often underlie issues in the query or storage layers and are critical to VDBMS robustness.

\noindent\textbf{Index Construction and Storage Issues.} 
Errors in building and maintaining index structures often lead to stale results or incomplete recall during search. 
Failures in this category often stem from \textbf{\textit{index construction error}}, where improper initialization, incorrect parameter configurations, or flawed data handling procedures result in incomplete or invalid index structures. Equally influential is \textbf{\textit{index update not synchronized}}, a condition in which updates to the underlying data are not correctly propagated to the index, leading to stale entries and inconsistent search outcomes. 


\begin{insightbox}
For VDBMS testing, it is essential to validate that index structures are properly initialized, configured, and populated. Tests should also cover data updates and deletions to ensure index entries stay synchronized.
\end{insightbox}

\noindent\textbf{Index Usage Issues.} 
Bugs in this category typically reflect misuses of the index during query execution. Some problems stem from \textbf{\textit{parameter misconfigurations}}, where inappropriate settings for parameters such as search depth or probe count result in degraded accuracy or unnecessary performance overhead. Others involve \textbf{\textit{data computation errors}}, which can cause the system to return incomplete or misleading results. These issues do not compromise the structural integrity of the index but significantly undermine its utility during runtime.



\subsubsection{Configuration}
A total of 387 bugs (26.5\% of all cases) stem from configuration issues, making it one of the most significant sources of failure. As shown in \autoref{fig:classification-configuration}, a large portion involves \textbf{\textit{environment configuration errors}}, such as mismatches between documentation and actual API behavior, library or runtime incompatibilities, and incorrect dependency setups across deployment platforms.
Another cause is \textbf{\textit{logging-related problems}}, where missing, unclear, or misleading log messages obscure root causes and hinder debugging.
These bugs are particularly challenging due to their diffuse nature: they often arise not from a single module but from complex interactions among system components, external tools, and user environments. This highlights the need for holistic testing, tighter integration between code and tooling, and better alignment between documentation and actual behavior.





\subsection{RQ3: Fix Strategies.}
We identify 12 representative fix strategies from an analysis of VDBMS bug-fixing commits. Each strategy reflects how developers resolve bugs by targeting configuration, code logic, data handling, or environment settings. \autoref{tab:fix-strategies} summarizes their distribution across four key areas: \textbf{Environment}, \textbf{Data}, \textbf{Program}, and \textbf{API}. We further group and analyze these strategies to understand their frequency and use cases.


\input{Tables/fix-strategy}
\input{Tables/RQ4-1}



\subsubsection{Environment} 
Fix strategies targeting the environment layer account for a substantial portion of all observed cases (239 in total). These are mainly used to resolve misconfigurations, compatibility issues, or incorrect setup procedures. The most common strategy is \textit{\textbf{updating configuration files or instructional materials}} (134 cases), which includes correcting default templates, adding missing setup steps, or clarifying deployment guides. Another frequent approach is \textit{\textbf{modifying environment variable values}} (41 cases) to fix path errors, resource visibility issues, or to enable or disable specific runtime behaviors. \textit{\textbf{Upgrading versions}} (30 cases) typically addresses library incompatibilities, outdated dependencies, or deprecation warnings. Finally, \textit{\textbf{modifying dependency configurations}} (34 cases) involves adding missing packages, adjusting version constraints, or removing conflicting dependencies. These changes are usually made through files such as \texttt{requirements.txt}, \texttt{poetry.lock}, or Dockerfiles.

\subsubsection{Data} 
Fix strategies at the data layer mainly fall into two categories. The first involves \textit{\textbf{modifying or adding data processing logic}} (40 cases), such as correcting preprocessing errors or adding missing normalization steps in ingestion pipelines. The second addresses \textit{\textbf{modifying data default values or initialization}} (46 cases), which often includes adjusting placeholder values, setting appropriate vector dimensions, or ensuring proper initialization of data fields to prevent runtime exceptions or incorrect computations.

\subsubsection{Program}
Program-level fix strategies are the most prevalent, addressing 1,079 bugs by modifying core logic to fix semantic errors, complete missing functionality, and handle edge cases. \textit{\textbf{Fixing or completing program logic}} (706 cases), which includes correcting control flow, adding missing conditional branches, or fixing flawed computations. Developers also often \textit{\textbf{add validation and safeguard mechanisms}} (188 cases) to prevent runtime exceptions and enforce correctness, such as checks for null values, vector dimensions, or operation preconditions. Other strategies include \textit{\textbf{removing redundant logic}} (60 cases), often left over from earlier development or refactoring, and \textit{\textbf{modifying parameter values}} (54 cases) to adjust thresholds, batch sizes, or resource limits. In performance-critical paths, \textit{\textbf{adjusting memory allocation strategies}} (71 cases) helps avoid out-of-memory errors and improve efficiency, particularly during large-scale vector operations.

\begin{insightbox}
Many program-level bugs in VDBMS stem from logic and edge-case errors that are hard to detect with standard unit tests. 
\end{insightbox}


\subsubsection{API}
Bugs related to incorrect or outdated API usage are addressed through a single but important strategy: \textit{\textbf{adjusting API usage}} (45 cases). These fixes typically involve modifying invocation methods, correcting argument formats, or reordering dependent function calls. Such issues are often triggered by breaking changes in upstream libraries or misuse of internal interfaces within the VDBMS engine.
To mitigate such issues, it is essential to strengthen interface contracts and improve change management practices. Effective measures include enforcing version checks, monitoring deprecation warnings, and isolating internal APIs from external exposure, especially in fast-evolving codebases.


==> Tables/RQ4-2.tex <==
\begin{table*}[h!]
\centering
\caption{Distribution of fix strategies across 15 vector databases.}
\resizebox{\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule[1.2pt]
\textbf{VecDB} & \multicolumn{12}{c}{\textbf{Fix Strategy}} & \textbf{Total} \\
\cmidrule(lr){2-13}
\textbf{} & \textbf{Upgrade} & \textbf{Dependencies} & \textbf{Env Vars} & \textbf{Config Files} & \textbf{Data Logic} & \textbf{Data Defaults} & \textbf{Code Logic} & \textbf{Params} & \textbf{Memory} & \textbf{Validation} & \textbf{Remove Logic} & \textbf{API Usage} & \textbf{} \\
\midrule
Faiss      & / & / & 77.8\% & / & 11.1\% & / & / & / & / & 11.1\% & / & / & 9 \\
Milvus     & 1.1\% & 0.6\% & 0.3\% & 3.3\% & 2.5\% & 2.8\% & 59.8\% & 4.7\% & 7.2\% & 10.7\% & 5.0\% & 2.2\% & 363 \\
Qdrant     & / & 7.4\% & 14.8\% & 3.7\% & / & 3.7\% & 44.4\% & / & 7.4\% & 18.5\% & / & / & 27 \\
Chroma     & 2.2\% & 14.0\% & 9.7\% & 6.5\% & 4.3\% & 2.2\% & 45.2\% & / & 3.2\% & 9.7\% & 2.2\% & 1.1\% & 93 \\
Annoy      & / & / & / & / & / & / & 100.0\% & / & / & / & / & / & 1 \\
Weaviate   & 2.2\% & 1.1\% & 1.1\% & 7.6\% & 2.2\% & / & 43.5\% & / & 8.7\% & 32.6\% & / & 1.1\% & 92 \\
txtai      & / & / & / & 40.0\% & / & / & / & / & / & 20.0\% & / & 40.0\% & 5 \\
Deep Lake  & 0.6\% & 1.2\% & / & 13.0\% & 3.0\% & 1.8\% & 55.0\% & 3.6\% & 4.7\% & 11.8\% & 1.2\% & 4.1\% & 168 \\
Vespa      & 2.6\% & 0.3\% & 0.9\% & 6.7\% & 0.9\% & 7.5\% & 46.4\% & 5.2\% & 3.2\% & 14.8\% & 8.1\% & 3.5\% & 348 \\
LanceDB    & 6.6\% & 9.2\% & 1.3\% & 13.2\% & 15.8\% & / & 39.5\% & 5.3\% & 1.3\% & 7.9\% & / & / & 76 \\
Marqo      & 1.9\% & 1.9\% & 5.7\% & 12.3\% & / & 2.8\% & 53.8\% & 4.7\% & 1.9\% & 11.3\% & 2.8\% & 0.9\% & 107 \\
Hnswlib    & / & / & 16.7\% & 16.7\% & / & / & 33.3\% & / & 16.7\% & 16.7\% & / & / & 6 \\
Usearch    & 2.6\% & / & 2.6\% & 21.1\% & 5.3\% & / & 39.5\% & 2.6\% & 2.6\% & 2.6\% & / & 21.1\% & 38 \\
pgvecto.rs & 3.5\% & 2.7\% & 6.2\% & 24.8\% & 1.8\% & 0.9\% & 36.3\% & 3.5\% & 7.1\% & 2.7\% & 6.2\% & 4.4\% & 113 \\
Voyager    & / & 5.9\% & / & 5.9\% & / & / & 23.5\% & / & / & 64.7\% & / & / & 17 \\
\bottomrule[1.2pt]
\end{tabular}
\end{threeparttable}}
\label{tab:rq4-2}
\end{table*}

